SmartSAGE: Training Large-scale Graph Neural Networks using In-Storage Processing Architectures

Graph neural networks (GNNs) can extract features by learning both the representation of each objects (i.e., graph nodes) and the relationship across different objects (i.e., the edges that connect nodes), achieving state-of-the-art performance in various graph-based tasks. Despite its strengths, utilizing these algorithms in a production environment faces several challenges as the number of graph nodes and edges amount to several billions to hundreds of billions scale, requiring substantial storage space for training. Unfortunately, state-of-the-art ML frameworks employ an in-memory processing model which significantly hampers the productivity of ML practitioners as it mandates the overall working set to fit within DRAM capacity. In this work, we first conduct a detailed characterization on a state-of-the-art, large-scale GNN training algorithm, GraphSAGE. Based on the characterization, we then explore the feasibility of utilizing capacity-optimized NVM SSDs for storing memory-hungry GNN data, which enables large-scale GNN training beyond the limits of main memory size. Given the large performance gap between DRAM and SSD, however, blindly utilizing SSDs as a direct substitute for DRAM leads to significant performance loss. We therefore develop SmartSAGE, our software/hardware co-design based on an in-storage processing (ISP) architecture. Our work demonstrates that an ISP based large-scale GNN training system can achieve both high capacity storage and high performance, opening up opportunities for ML practitioners to train large GNN datasets without being hampered by the physical limitations of main memory size.

==> tex/evaluation.tex <==
\section {Evaluation} 
\label{sect:evaluation}

We explore four design points: two baseline architectures, 1) CPU-GPU
without caching, 2) a CPU-GPU with static GPU embedding cache, and
two design points from our proposal, 
3) our straw-man architecture \emph{without} pipelining,
	and 4) \proposed \emph{with} pipelining. Note that \proposed
	\emph{does not change the algorithmic properties of
	stochastic gradient descent (SGD) training} so the total training iterations required
		to reach a given target CTR accuracy is identical between baseline
		and \proposed.

\subsection{Latency Breakdown}
\label{sect:eval_latency_breakdown}

Before discussing end-to-end performance of \proposed, we analyze its efficacy
in addressing baseline architecture's bottlenecks.
\fig{fig:eval_latency_breakdown} shows a latency breakdown of our studied
workloads.  As discussed in \sect{sect:motivation_caching}, our two baselines
spend significant fraction of training time in conducting the memory bound
embedding layer training at the low throughput CPU memory. While storing hot
entries in GPU's embedding cache does help alleviate the bottlenecks of
CPU-side training (with larger caches generally helping reduce CPU-side
		training time), it fails to overcome the fundamental limitations of slow
CPU memory as any embedding table accesses that miss in the GPU cache must be
routed to CPU memory to conduct not just the embedding gathers (forward
		propagation) but more importantly the highly memory bound gradient
duplication/coalescing followed by scatter updates during backpropagation
(\fig{fig:recsys_training}(b), \fig{fig:baseline_vs_caching_flow}(b)).  As
shown in \fig{fig:eval_latency_breakdown}(b), \proposed substantially reduces
latency because the memory intensive embedding layer training is always
conducted over our high-bandwidth GPU scratchpad. In \proposed, the only time
CPU memory is accessed is when the embeddings to be prefetched into GPU
scratchpad are [Collect]ed and when the updated models are evicted and
[Insert]ed into CPU embedding tables. While these two stages do incur
high latency within \proposed's cache management step, the absolute time
spent in interacting with the CPU memory is significantly reduced compared to
the baseline static caching, all thanks to
our GPU scratchpad.
		
\subsection{Performance}
\label{sect:eval_perf}

\begin{figure}[t!] \centering
    \subfloat[]
    {
        \includegraphics[width=0.465\textwidth]{./fig/eval_breakdown_baseline.pdf}
    }
    \vspace{-0em}
    \subfloat[]
    {
    \includegraphics[width=0.465\textwidth]{./fig/eval_breakdown_ours.pdf}
    }
    \vspace{0em}
    \caption{
		Latency breakdown of (a) baseline CPU-GPU without caching ($0\%$) and with static GPU
			embedding cache (sized to accommodate top $2-10\%$ of hot entries in CPU embedding tables). 
			In (b), \proposed is broken down into its per-stage pipeline latency. Note that the scale
			in (a) and (b) are different ($0-200$ ms in (a) vs. $0-70$ ms in (b)).
    }
    \label{fig:eval_latency_breakdown}
		\vspace{-1.3em}
\end{figure}

\fig{fig:eval_speedup} shows \proposed's  end-to-end speedup. Across all
the data points we explore, \proposed achieves an average $2.8\times$ (max $4.2\times$)
	speedup vs. static caching, with the magnitude of performance improvement gradually
	reducing as input traces exhibit higher locality. This is expected because the more locality
	a given dataset contains, the lightweight static embedding cache design could cost-effectively
	absorb the majority of embedding table accesses. Nonetheless, even under a high locality
	workload scenario, \proposed achieves $1.6-1.9\times$ speedup, demonstrating its robustness.
	Interestingly, our straw-man without pipelining
	also provides meaningful speedup vs. static caching as it still helps reduce the number of
	gradient scatters to the CPU embedding tables, highlighting the benefits of dynamic caching vs.
	static. 

\subsection{Energy-Efficiency}
\label{sect:eval_energy}

\proposed is a purely software-based architecture
demonstrated over existing hardware/software stack.  To
measure system-level power consumption, we utilize \texttt{pcm-power}~\cite{pcm_power} for CPU's
socket-level power consumption and NVIDIA's \texttt{nvidia-smi}~\cite{nvidia_smi} for GPU power
consumption. The aggregated power is multiplied with execution time to derive energy
consumption. As depicted in \fig{fig:eval_energy}, 
\proposed's significant training time reduction directly
	translates into energy-efficiency improvements.

	\begin{figure}[t!] \centering
    \includegraphics[width=0.47\textwidth]{./fig/eval_speedup.pdf}
    \caption{
				End-to-end performance speedup (normalized to static cache).
        }
        \vspace{-0.5em}
        \label{fig:eval_speedup}
\end{figure}


\begin{figure}[t!] \centering
    \includegraphics[width=0.47\textwidth]{./fig/eval_energy.pdf}
    \caption{
				Energy consumption of static cache vs. \proposed.
        }
        \vspace{-1.3em}
        \label{fig:eval_energy}
\end{figure}


\subsection{Implementation Overhead}
\label{sect:eval_overhead}

As discussed in \sect{sect:proposed_implementation},
\proposed requires the Storage array within our GPU scratchpad to at least be
large enough to accommodate all the embeddings gathered across the six input mini-batches
currently falling under the sliding window. Under our default \recsys model
configuration, in the worst case where none of the IDs within the sliding window overlap with each other, this amounts to (number of tables $\times$ number of gathers per table
		$\times$ mini-batch size $\times$ embedding vector size) $\times$ (number of concurrent mini-batches) = ($8\times20\times2048\times128\times4$ Bytes)$\times$$6$ = $960$ MB of Storage space
provisioned for holding not-to-be-evicted embeddings. In reality however, the \emph{active} 
working set to actually hold is significantly smaller as many of the IDs gathered within
the sliding window become hits.
				In addition, the Hit-Map also incurs an additional $<$$1$ GB of memory space with other 
				miscellaneous data structures accounting for $<$$300$ MB, amounting to 
				an aggregate $<4$ GB of additional GPU side memory allocations under \proposed.


\begin{figure}[t!] \centering
    \subfloat[]
    {
        \includegraphics[width=0.475\textwidth]{./fig/sensitivity_emb_dim.pdf}
    }
    \vspace{-0em}
    \subfloat[]
    {
    \includegraphics[width=0.475\textwidth]{./fig/sensitivity_lookups.pdf}
    }
    \vspace{-0em}
    \caption{
		\proposed sensitivity to (a) embedding vector dimension size ($64$/$128$/$256$), (b) number of embedding table lookups ($1$/$20$/$50$).
    }
    \label{fig:eval_sensitivity}
		\vspace{-1.3em}
\end{figure}


\subsection{Sensitivity}
\label{sect:sensitivity}

 This section evaluates \proposed's  robustness to
\recsys model configuration or design parameters
 of \proposed. 


{\bf Embedding vector dimension.} Although our default embedding vector
dimension is sized at $128$, several prior work employs smaller~\cite{recnmp}
or larger~\cite{mudigere2021high,youtube_recsys} dimension sizes in their \recsys. \fig{fig:eval_sensitivity}(a)
shows \proposed's speedup when sweeping the embedding dimension size from
$64$ to $256$. In general, the performance benefits of \proposed remains intact
across embedding dimension size with larger speedups achieved when the dimension
size gets larger. This is because larger embeddings incur an even higher memory
bandwidth pressure, rendering baseline to suffer more while \proposed's scratchpad
providing higher performance benefits.

{\bf Number of embedding table lookups.} 
\fig{fig:eval_sensitivity}(b) summarizes
the speedup \proposed achieves when the number of
embedding table gathers are swept from $1$ to $50$. 
As the number of lookups are increased to $50$, the embedding layer
causes an even more severe performance bottlenecks due to its increase
in memory traffic. Consequently, \proposed
achieves an even higher speedup with an average $3.7\times$ (max $5.6\times$). At the other end of the spectrum, we experiment an embedding table 
lookup size of $1$ which makes the \recsys model suffer less from the embedding layers. \proposed still performs better than our two baselines albeit with less improvements in performance. 
Generally, \proposed is shown to be highly robust 
across a wide range of embedding table lookup sizes.

{\bf Cache replacement policy, MLP-intensive \recsys models, etc.} In addition
to the aforementioned sensitivity studies, we also tested \proposed's
robustness under various other design points: 1) changing the GPU scratchpad's
replacement policy from our default LRU (least-recently-used) policy to a
random eviction or LFU (least-frequently-used) policy, 2) evaluating the
effectiveness of \proposed under more MLP-intensive (and less embedding
		intensive) models, 3) training under larger or smaller batch sizes, etc.
		In general, we confirm \proposed's robustness across a wide range of
		sensitivity studies. We omit the results for brevity.


\subsection{Training Cost Reduction vs. Multi-GPUs}
\label{sect:eval_cost_new}

We now discuss \proposed's benefits in reducing \recsys training cost.
	Training cost estimates are based on AWS EC2 pricing for P3 instances
		containing NVIDIA V100 GPUs (\tab{tab:tco}). \proposed does not
		change the training algorithm so the total number of training iterations
		required to reach the same level of \recsys algorithmic accuracy are
		identical between \proposed and the $8$ GPU system.  As such, we evaluate
		the training costs for the evaluated systems over $1$ million training
		iterations.  The $8$ multi-GPU  system partitions the embedding tables
		across $8$ GPUs' HBM for model-parallel training of embeddings while the
		backend MLP layers are trained using data-parallelism, enabling end-to-end
		``GPU-only'' training.  Despite using $8$ GPUs, however, the multi-GPU
		system can only reduce $29\%$/$40\%$/$64\%$/$66\%$ of training time vs.
		\proposed for high/medium/low/random datasets.  Consequently, \proposed
		consistently achieves significant training cost reduction with an average
		$4.0\times$ (maximum $5.7\times$) savings, with more cost
		savings achieved with higher locality.


\begin{table}[t!]
  \caption{Training cost of ScratchPipe vs. multi-GPU with $8$ V100 GPUs. %Cost estimates are based on AWS EC2 pricing for P3 instances, assuming $1$ million training iterations.
  }
  \centering
\footnotesize
\scalebox{0.82}{
  \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \textbf{Dataset} & \textbf{System} & \textbf{AWS Instance} & \textbf{Price/hr} & \textbf{Iter. Time} & \textbf{1M Iter. Cost} \\ \hline
      \hline\hline
      \multirow{2}{*}{Random} & ScratchPipe   &   p3.2xlarge   & \$ 3.06  & 47.82 ms & \textbf{\$ 40.64} \\  \cline{2-6}
                              & 8 GPU         &   p3.16xlarge  & \$ 24.48 & 16.22 ms & \$ 110.3  \\  \hline\hline
      \multirow{2}{*}{Low}    & ScratchPipe   &   p3.2xlarge   & \$ 3.06  & 44.70 ms & \textbf{\$ 37.99}  \\  \cline{2-6}
                              & 8 GPU         &   p3.16xlarge  & \$ 24.48 & 16.12 ms & \$ 110.2 \\  \hline\hline
      \multirow{2}{*}{Medium} & ScratchPipe   &   p3.2xlarge   & \$ 3.06  & 29.68 ms & \textbf{\$ 25.23} \\  \cline{2-6}
                              & 8 GPU         &   p3.16xlarge  & \$ 24.48 & 17.82 ms & \$ 121.2 \\  \hline\hline
      \multirow{2}{*}{High}   & ScratchPipe   &   p3.2xlarge   & \$ 3.06  & 26.34 ms & \textbf{\$ 22.39} \\  \cline{2-6}
                              & 8 GPU         &   p3.16xlarge  & \$ 24.48 & 18.61 ms & \$ 126.6 \\  \hline
  
  \end{tabular}
}
\vspace{-1.5em}
\label{tab:tco}
\end{table}


\subsection{Discussion}
\label{sect:eval_scalability}

{\bf Applicability of single CPU-GPU ScratchPipe.}
Recent literature from Facebook elaborate on the scale of their deployed
	RecSys model size, exhibiting upto $100\times$ difference in number of
		embedding tables per model~\cite{mudigere2021software,deeprecsys}.   Specifically, RecSys models for
			content filtering are known to be smaller sized than those for
				ranking~\cite{dlrm:arch}, enabling the overall memory footprint to fit
					within a single-node's CPU memory capacity.  Given content filtering's
						wide applicability across various web-based applications
						(e.g., filter down movies/news/products to recommend to user), we expect our
						single CPU-GPU ScratchPipe to be widely applicable as-is over a
						variety of use cases, providing significant reduction in TCO vs. multi-GPUs.  

{\bf ScratchPipe for multi-GPU training.} In
\sect{sect:eval_cost_new}, we demonstrated the advantages of employing single GPU
	ScratchPipe in terms of TCO reduction vs. multi-GPU systems. While this paper
		focuses on the single GPU based ScratchPipe design point, for the
		completeness of our study, we nonetheless discuss the practicality of
		extending our solution for multi-GPU systems below.  A popular approach in
		partitioning and parallelizing RecSys among multi-GPUs is to employ
		table-wise model-level parallelism (i.e., partition distinct set of
				embedding tables across different GPUs) and have each GPU locally go
		through the embedding layer forward/backpropagation as usual, i.e., each
		partitioned embedding table is locally treated as an \emph{independent}
	embedding table from each GPU's perspective~\cite{mudigere2021high}. ScratchPipe is designed to handle GPU cache management in a per embedding table granularity,
	 i.e., RecSys with $N$ embedding tables will have $N$ instance of
		 ScratchPipe's cache manager module instantiated.  As existing
		 model-parallelization for embeddings are carefully designed to
		 enable each GPU to locally handle forward and backpropagation of
		 embedding layers independently with minimum communication, there
		 is no further inter-GPU RAW hazards or any reordering of embedding lookup
		 indices
		 required for correctness and we expect that ScratchPipe can be
		 seamlessly integrated for multi-GPU training.
That being said, while extending ScratchPipe for multi-GPU systems is a viable
design point to explore, it is likely not going to be cost-effective 
in terms of TCO reduction. This is because
parallelizing the DNNs over multi-GPUs only
provides incremental end-to-end performance improvements
(i.e., even with a single GPU, the DNNs are not the
most crucial bottleneck, \fig{fig:eval_latency_breakdown}). 
Consequently, ScratchPipe over multi-GPUs can severely underutilize the
abundant GPU compute throughput, leading to lower training
cost savings.
A detailed,
quantitative evaluation of such is beyond the scope of this paper
and we leave it as future work. 

				







==> tex/motivation.tex <==
\section{Motivation} 
\label{sect:characterization}
\old{
In this section, we conduct a detailed characterization on the
locality in embedding table accesses which the 
baseline hybrid CPU-GPU system can exploit for \recsys training
performance improvements. 
training performance, root-causing its performance bottlenecks.  
as discussing the benefits of utilizing caching for training system performance
improvements.
}

\subsection{Locality in Embedding Layer Training}
\label{sect:motivation_locality}

In \fig{fig:motivation_locality}, we show the (sorted) access count of  
embedding table entries in various real-world \recsys datasets.
The embedding table accesses generally exhibit a power-law
distribution where a small subset of table entries receive very high access
frequency while the remaining entries receive only a small number of accesses.
Such long-tail phenomenon  is not surprising as it is typically the
case where a large fraction of \recsys users are interested in a small portion
of the most popular items (e.g., popular products in Amazon or most watched
		movies in Netflix). While the magnitude of locality  is highly dependent on where the \recsys
		model is being deployed for (e.g., in Criteo Ad Labs, $2\%$ of the
				embeddings account for more than $80\%$ of all accesses whereas
				for Alibaba User dataset, $2\%$ of embeddings ``only'' account
				for $8.5\%$ of traffic), we generally observe that \recsys 
		datasets indeed exhibit the power-law distribution with a very long-tail.

Unfortunately, the baseline hybrid CPU-GPU is not designed to leverage
the unique locality properties of embedding layers~\cite{tcasting}.
\fig{fig:baseline_vs_caching_flow}(a) shows the key stages of forward and
backpropagation under baseline CPU-GPU. As depicted,  the memory bandwidth limited
embedding gather and gradient scatter operations are all conducted over the
slow CPU memory, so the end-to-end training time is primarily
bottlenecked on the CPU-side training of embedding layers, consuming
significant portion of training time
(\fig{fig:motivation_latency_breakdown}).


\subsection{Software-Managed Embedding Caches}
\label{sect:motivation_caching}

	
			\begin{figure}[t!] \centering
    \includegraphics[width=0.48\textwidth]{./fig/latency_breakdown_baseline.pdf}
    \caption{
      Training time broken down based on where key stages are executed (CPU vs. GPU).
				The software-managed GPU embedding cache is sized to store the
				most-frequently-accessed top $2\%$/$10\%$ of embedding table entries.
				Random/Low/Medium/High in the x-axis indicates the magnitude of locality
				inherent in the \recsys dataset we study.
				\sect{sect:methodology} details our methodology.
        }
        \label{fig:motivation_latency_breakdown}
\end{figure}


Given the power-law distribution of embedding table accesses, an effective
mechanism to exploit such locality is to incorporate a small GPU
\emph{embedding cache} (managed in fast GPU DRAM) that can help reduce the
embedding gather/gradient scatter traffic to CPU memory.
\fig{fig:baseline_vs_caching_flow}(b) provides an overview of \recsys training
under a CPU-GPU system enhanced with a software-managed GPU embedding cache.
The key data structures of such software-level cache (e.g., tag, data, other metadata)
	as well as its cache controller module
are all implemented and managed in software
	over GPU memory using CUDA~\cite{cuda}. In 
	terms of cache management policies, we
assume the \emph{static} cache architecture suggested by Yin et
al.~\cite{ttrec} where the most-frequently-accessed embeddings (i.e., the
top-$N$ leftmost table entries in \fig{fig:motivation_locality}) are chosen
for caching in GPU DRAM without getting evicted throughout the entire \recsys
training process. 
\fig{fig:motivation_latency_breakdown} shows the normalized
end-to-end training time broken down based on where the key stages of training
is executed.  We make several important observations from this experiment.
First, the static GPU embedding cache noticeably reduces the time spent in the
memory bandwidth limited embedding layer training. This is because of the hot
embeddings hitting in the GPU embedding cache, which helps filter out the
number of embedding table accesses serviced by the CPU memory.  Unfortunately,
			 there is still a non-negligible amount of time spent in servicing the
			 (embedding cache missed) embedding gathers and gradient scatter
			 operations over CPU memory, averaging at $77\%$ to $94\%$ of
training time. In particular, the backpropagation of embedding layers
	corresponding to the \emph{missed IDs} (the rightmost two black stages in
			\fig{fig:baseline_vs_caching_flow}(b))	invoke memory bandwidth
		limited gradient duplication/coalescing/scatters over the slow CPU
		memory, causing serious latency overheads. 
	 On
		average, the static GPU embedding cache suffers from $12\%$ (high locality dataset) to
			$91\%$ (low locality dataset) cache miss rates, all of which must be serviced from CPU
			embedding tables.
		
	\begin{figure}[t!] \centering
        \includegraphics[width=0.48\textwidth]{./fig/cache_hit_rate_terabyte.pdf}
    \caption{
			Static GPU embedding cache hit rate as a function of cache size, for
				(a) Alibaba, (b) Kaggle Anime, (c) MovieLens, and (d) Criteo. $100\%$ cache size
				means the GPU embedding cache is large enough to fully cache the entire embedding
				tables within GPU's local high-bandwidth memory. 
        }
        \vspace{-1.25em}
    \label{fig:motivation_cache_hitrate}
\end{figure}


	One might argue that a \emph{larger} GPU embedding cache could
	potentially absorb the majority of traffic to CPU memory and enable the
	performance of CPU-GPU to reach that of a ``GPU-only'' system (i.e., the
			high-bandwidth GPU memory stores \emph{all} embedding tables, allowing
			embedding layers to be trained at  GPU memory speed).
	\fig{fig:motivation_cache_hitrate} plots the improvements in GPU embedding
	cache hit rate as we cache a larger fraction of CPU embedding tables. For
	datasets like Criteo, a small fraction of hot embedding table entries exhibit
	extremely high locality (\fig{fig:motivation_cache_hitrate}(d)).
	Consequently, having larger embedding caches provide only incremental
	improvements in further absorbing CPU memory traffic.  Conversely, for
	datasets with low locality 
	(\fig{fig:motivation_cache_hitrate}(a)), achieving $>$$90\%$ cache hit rates
	would require more than $65\%$ of the embedding table entries to be cached in
	GPU memory.  Given state-of-the-art \recsys require TB-scale memory
	capacity, caching such high proportion of embedding tables is an impossible
	design point to pursue given the ``meager'' tens of GBs of GPU memory.

\subsection{Our Goal: Training Embedding Layers at GPU Memory Speed}
\label{sect:motivation_goal}

Our characterization root-caused the memory bandwidth limited embedding
layer training  as a key limiter in \recsys
training's performance. Caching most-frequently-accessed, hot embeddings inside
high-bandwidth GPU memory could alleviate the performance penalties of sparse
embedding gathers and gradient scatters, but the limited GPU memory capacity
makes it impossible to fully capture the active working set of embedding
tables. This makes GPU embedding caches to still suffer from the latency
overhead of bringing in the missed embeddings from CPU memory, which sits on
the critical path of \recsys training and hurting performance.  
A key
	objective of our study is to develop a GPU embedding cache that
		is able to intelligently store (and evict) not just the current but also
		\emph{future} embedding table accesses such that its active working set 
		is ``always'' available within GPU memory by the time embedding layer
		training is initiated. This would allow the training of embedding
		layers to occur at the speed of high-throughput GPU memory, drastically
		improving the performance of end-to-end \recsys training. 

